Minority-spin conducting states in Fe substituted pyrite CoS$_2$

There has been a longstanding debate whether the pyrite CoS$_2$ or its alloys with FeS$_2$ are half metallic. We argue using first principles calculations that there is a finite occupation of minority-spin states at the Fermi level throughout the series Co$_{1-x}$Fe$_x$S$_2$. Although the exchange-correlation functional influences the specifics of the electronic structure, we observe a similar trend with increasing Fe concentration in both LDA and GGA calculations. Specifically, even as band filling is decreased through Fe substitution, the lowest-lying conduction band in the minority-spin channel broadens such that these states keep getting lowered relative to the Fermi level, which is contrary to the expectations from a rigid band picture. Furthermore, the exchange splitting decreases as more Co atoms are replaced by Fe, and this again brings the minority-spin states closer to the Fermi level. These two mechanisms, in conjunction with the experimental observation that minority-spin bands cross the Fermi level in stoichiometric CoS$_2$, indicate that minority-spin charge carriers will always be present in Co$_{1-x}$Fe$_x$S$_2$.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\usepackage{caption}
\usepackage{indentfirst}

